TriCoLo: Trimodal Contrastive Loss for Text to Shape Retrieval

Text-to-shape retrieval is an increasingly relevant problem with the growth of 3D shape data. Recent work on contrastive losses for learning joint embeddings over multimodal data has been successful at tasks such as retrieval and classification. Thus far, work on joint representation learning for 3D shapes and text has focused on improving embeddings through modeling of complex attention between representations, or multi-task learning. We propose a trimodal learning scheme over text, multi-view images and 3D shape voxels, and show that with large batch contrastive learning we achieve good performance on text-to-shape retrieval without complex attention mechanisms or losses. Our experiments serve as a foundation for follow-up work on building trimodal embeddings for text-image-shape.

==> sections/figtables/tab-results-clip-simplified-with-c13.tex <==
\begin{table}
\caption{\todo{the chairs+tables results seems redundant}Comparison of text to shape retrieval performance using CLIP-based models against prior work on the test set. We report the recall rate (RR@1, RR@5) and NDCG@5 as percentages. It can be seen that zero-shot CLIP has relatively good performance considering that it has not been trained on the Text2Shape~\cite{chen2018text2shape} `chairs and tables' dataset.  Training an MLP to project the CLIP embeddings (CLIP-MLP) drastically improves the retrieval performance, but still underperforms our \trimodiv model.}
\vspace{-5pt}
\centering
\resizebox{\linewidth}{!}
{
\begin{tabular}{@{}rrrrr@{}}
\toprule
 & \multicolumn{2}{c}{chairs+tables (test)} & \multicolumn{2}{c}{ShapeNet c13 (val)} \\
\cmidrule(l{0pt}r{2pt}){2-3}
\cmidrule(l{0pt}r{2pt}){4-5}
& RR@1 & RR@5 & RR@1 & RR@5 \\
\midrule
Text2shape[1]  & 0.40 & 2.37 & - & - \\
CLIP (ZS)[2] & 6.25 & 15.72 & 6.81 & 16.97 \\
Parts2Words (global) [3]  & 8.60 & 24.82 & - & - \\
Parts2Words (full) [3]  & 12.72 & 32.98 & - & - \\
CLIP[2]+ MLP & 8.22 & 24.19 & 9.52 & 27.51 \\  %
\bimodi (ours)  & 11.09 & 30.78 & 11.89 & 33.48 \\
\bimodv (ours)  & 8.93 & 26.71 & 9.48 & 29.22 \\
\trimodiv (ours) & 12.22 & 32.23 & 12.96 & 34.87 \\

\bottomrule
\end{tabular}
}
\vspace{-10pt}
\label{tab:retrieval-clip}
\end{table}

==> sections/figtables/tab-results-clip-simplified.tex <==
\begin{table}
\caption{Comparison of text to shape retrieval performance using CLIP-based models against prior work on the test set. We report the recall rate (RR@1, RR@5) and NDCG@5 as percentages. It can be seen that zero-shot CLIP has relatively good performance considering that it has not been trained on the Text2Shape~\cite{chen2018text2shape} `chairs and tables' dataset.  Training a MLP to project the CLIP embeddings (CLIP-MLP) drastically improves the retrieval performance, but still underperforms our \trimodiv model.}
\vspace{-5pt}
\centering
\resizebox{\linewidth}{!}
{
\begin{tabular}{@{}rrr@{}}
\toprule
test set & RR@1 & RR@5 \\
\midrule
Text2shape[1]  & 0.40 & 2.37 \\
CLIP[2] & 1.63 & 5.34 \\
Part2Word[3]  & 7.94 & 23.89 \\
CLIP[2]+ MLP & 8.22 & 24.19 \\  %
\bimodi (ours)  & 8.28 & 24.52 \\
\bimodv (ours)  & 8.73 & 26.10 \\
\trimodiv (ours) & \textbf{10.25} & 
\textbf{29.07} \\

\bottomrule
\end{tabular}
}
\vspace{-10pt}
\label{tab:retrieval-clip}
\end{table}
